The TLA+ Toolbox

We discuss the workflows supported by the TLA+ Toolbox to write and verify specifications. We focus on features that are useful in industry because its users are primarily engineers. Two features are novel in the scope of formal IDEs: CloudTLC connects the Toolbox with cloud computing to scale up model checking. A Profiler helps to debug inefficient expressions and to pinpoint the source of state space explosion. For those who wish to contribute to the Toolbox or learn from its flaws, we present its technical architecture.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{R. Monahan, V. Prevosto, J. Proen\c{c}a (Eds.): Formal\\
Integrated Development Environment 2019 (F-IDE 2019)\\
EPTCS 310, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.310.6}{10.4204/EPTCS.310.6}}
\pdfoutput=1

